Global AdS Picture of 1/2 BPS Wilson Loops

We study the holographic dual string configuration of 1/2 BPS circular Wilson loops in N=4 super Yang-Mills theory by using the global coordinate of AdS. The dual string worldsheet is given by the Poincare disk AdS_2 sitting at a constant global time slice of AdS_5. We also analyze the correlator of two concentric circular Wilson loops from the global AdS perspective and study the phase transition associated with the instability of annulus worldsheet connecting the two Wilson loops.

==> hyperbasics.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                         %
% This file is written by Tanmoy Bhattacharya <tanmoy@qcd.lanl.gov> and   %
% is in the public domain for what it is worth. It inserts \specials that %
% are interpreted by (a) the xhdvi hypertex dvi previewer, (b) nextstep   %
% HyperTeXview.app dvi previewer, and (c) the dvipdf driver               %
% For more info, see http://xxx.lanl.gov/hypertex/                        %
%                or  ftp://xxx.lanl.gov/pub/hypertex/index.html           %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                         %
% Only \hyperdef, \hyperref , \href , and \hname are user callable.       %
% Usage: \hyperdef\TeXcs{category}{name}{text}                            %
% Usage: \href{url}{text}                                                 %
% Usage: \hyperref{filename}{category}{name}{text}                        %
%   or   \hyperref\TeXcs{text}                                            %
%             where \TeXcs has been defined by a hyperdef.                %
%                                                                         %
%        Note: The token following \hyperref is expanded completely first.%
%              Really perverse forms like                                 %
%                \csname perverse\endcsname                               %
%              will give an error                                         %
%                                                                         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The following might be useful to other macros interfacing in.           %
% Usage: \hyper@nchor{name="#myname" href="#refer"}{text}                 %
% Usage: \hyperlink{target_name}{text}                                    %
% Usage: \hypertarget{myname}{text}                                       %
% In cases where there is a possibility of premature expansion use        %
%     \hyper@\hyperpr@ref instead of \hyperref                            %
% and \hyper@\hyperpr@def instead of \hyperdef                            %
% These macros increase enormously in size when expanded, but the expanded%
% token sequence always ends in \hyperpr@ref and \hyperpr@def respectively%
% Macro writers might want to make use of the macro \hyperv@rsion         %
% which is undefined in version 0 and is the version number otherwise     %
% \hyper@nique is exactly like \hyperdef except no special are written    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Save the current catcode of @ and redefine @ to be a letter
%
\expandafter\edef\csname hypers\string @fe\endcsname{\catcode
                                             `\noexpand @=\the\catcode`\@}%
\catcode`\@=11
%
% Check if the file is already included
%
% hack to allow \allowoncemore
\ifx\hyper@utoprocess\hyper@ndefined
\else
 \expandafter\hyper@utoprocess\fi
\ifx\hyperd@ne\hyper@ndefined
 \global\let\hyperd@ne=\relax
\else
 \hypers@fe
 \errhelp{hyperbasics.tex needs to be included only once outside
          of any {...} or \begingroup...\endgroup. You have tried to
          include it more than once. If the previous include was indeed
          outside any groupings, continue and all will be well.}%
 \errmessage{Input this file only once!}%
 \expandafter\endinput\fi
%
% Version number
%
\def\hyperv@rsion{12}%
%
% Check and input a previous .hrf file if it exists
%
\newread\hyperf@le
\def\hyperf@lename{\jobname.hrf}%
\immediate\openin\hyperf@le\hyperf@lename\relax
\ifeof\hyperf@le\relax
 \immediate\closein\hyperf@le\relax
\else
 \immediate\closein\hyperf@le\relax
 \input \hyperf@lename
\fi
%
% Open a new .hrf file
%
\newwrite\hyperf@le
\immediate\openout\hyperf@le\hyperf@lename
%%%%
% MAIN SECTION
%%%%
%
% define a token register
%
\newtoks\hypert@ks
%
% Define a convenient macro to hold the character #
%
\edef\hypert@mp{\catcode`\noexpand\%=\the\catcode`\%}
\catcode`\%=12
\def\hyperp@rcent{%}
\hypert@mp
\edef\hypert@mp{\catcode`\noexpand\#=\the\catcode`\#}%
\catcode`\#=12
\def\hyperh@sh{#}%
\hypert@mp
\let\hypert@mp=\relax
\let\hyper@nd=\relax
\def\hyperbl@nk{ }
\def\hyperstr@pquote#1"#2\hyper@nd{% Call \hyperstr@pquote..."\hyper@nd
   #1% #1 can not contain "
   \ifx\hyper@nd#2\hyper@nd% #2 cannot contain \hyper@nd and
                           % must end in " if non-empty
   \else\hyperp@rcent22\hyperstr@pquote#2\hyper@nd\fi}%
\def\hyperstr@pblank#1 #2\hyper@nd{% Call \hyperstr@pblank... \hyper@nd
   #1% #1 cannot contain a space
   \ifx\hyper@nd#2\hyper@nd% #2 canot contain \hyper@nd and
                           % and must end in blank if nonempty
   \else\hyperp@rcent20\hyperstr@pblank#2\hyper@nd\fi}
%
\long\def\hyper@nchor#1#2{\edef\hyperm@cro{html:<A #1>}%
                          \special\expandafter{\hyperm@cro}%
                          {#2}\special{html:</A>}}%
%
\def\hyper@atm@ning#1->#2\hyper@nd{#2}
\def\hyperlink{\protect\hyperlink@}
\def\hyperlink@{{\catcode\expandafter`\noexpand\#=12 
                 \catcode\expandafter`\noexpand\%=12 
                 \catcode\expandafter`\noexpand\~=12
                \expandafter}\hyperlink@@}
\def\hyperlink@@#1{\protect\hyperlink@@@{#1}}
\def\hyperlink@@@#1{\edef\hypert@mp{#1}%
               \edef\hypert@mp{\expandafter\hyper@atm@ning\meaning\hypert@mp
                               \hyper@nd}%
               \edef\hypert@mp{\expandafter\hyperstr@pquote%
                               \hypert@mp"\hyper@nd}%
               \edef\hypert@mp{\expandafter\expandafter\expandafter
                               \hyperstr@pblank\expandafter%
                               \hypert@mp\hyperbl@nk\hyper@nd}%
               \hyper@nchor{href=\expandafter"\hypert@mp"}}%
%
\def\hypertarget#1{\edef\hypert@mp{#1}%
               \edef\hypert@mp{\expandafter\hyper@atm@ning\meaning\hypert@mp
                               \hyper@nd}%
               \edef\hypert@mp{\expandafter\hyperstr@pquote%
                               \hypert@mp"\hyper@nd}%
               \edef\hypert@mp{\expandafter\expandafter\expandafter
                               \hyperstr@pblank\expandafter%
                               \hypert@mp\hyperbl@nk\hyper@nd}%
               \hyper@nchor{name=\expandafter"\hypert@mp"}}%
%
\def\hyperref{\afterassignment\hyperr@f\let\hyperp@ram}
\def\hyperr@f{\ifx\hyperp@ram{\iffalse}\fi
               \expandafter\expandafter\expandafter\hyperr@@
               \expandafter{%
              \else
               \iffalse}\fi
               \ifx\hyperp@ram\hyper@ndefined
                 \message{Undefined reference}%
                 \def\hyperp@r@m{{}{undefined}{}}%
               \else
                 \edef\hyperp@r@m{\hyperp@ram}%
               \fi
               \expandafter\expandafter\expandafter\hyperr@@
               \expandafter\hyperp@r@m
              \fi}%
% refer to #1, \hyperh@sh#2.#3 or #1\hyperh@sh#2.#3
% depending on what is blank/nonblank
\def\hyperr@@#1#2#3{\ifx\hyper@ndefined#1\hyper@ndefined
                    \hypert@ks\expandafter{\hyperh@sh#2.#3}%
                    \else
                     \ifx\hyper@ndefined#2#3\hyper@ndefined
                      \hypert@ks{#1}%
                     \else
                      \def\hypert@mp{#1}%
                      \hypert@ks\expandafter\expandafter\expandafter
                      {\expandafter\hypert@mp\hyperh@sh#2.#3}%
                     \fi
                    \fi
                    \expandafter\hyperlink\expandafter{\the\hypert@ks}}%
%
% \def\hyperREF#1{\hyperlink{#1}}% % Disabled as per pg's suggestion
%
\def\hyperdef#1#2#3{{\escapechar=`\\\relax
                     \edef\hyper@t@mp@{\hyperstr@pquote#2.#3"\hyper@nd}%
                     \expandafter\ifx\csname hyperd@\meaning\hyper@t@mp@
                     \endcsname
                     \relax
                     \expandafter\gdef\csname hyperd@\meaning\hyper@t@mp@
                     \endcsname{}%
                     \gdef#1{{}{\hyperstr@pquote#2"\hyper@nd}%
                               {\hyperstr@pquote#3"\hyper@nd}}%
                     \immediate\write\hyperf@le{\def\noexpand#1{{}%
                        {\noexpand\hyperstr@pquote#2"\noexpand\hyper@nd}%
                        {\noexpand\hyperstr@pquote#3"\noexpand\hyper@nd}}}%
                     \xdef\hyper@t@mp@{\global\let\noexpand\hyper@t@mp@=\relax
                                       \noexpand\hypertarget{\hyper@t@mp@}}%
                     \global\hypert@ks={\hyper@t@mp@}%
                     \else
                     \message\expandafter{\expandafter'\hyper@t@mp@' duplicate}%
		     \def\hyper@@tmp@{\hyperdef{#1}{#2}}%
		     \edef\hyper@@tmp@@{{#3@}}%
                     \global\let\hyper@t@mp@=\relax
                     \global\hypert@ks=\expandafter\expandafter
		     \expandafter{\expandafter\hyper@@tmp@\hyper@@tmp@@}%
                     \fi}\the\hypert@ks}%

\def\hyper@nique#1#2#3#4{{\escapechar=`\\\relax
                     \edef\hyper@t@mp@{\hyperstr@pquote#2.#3"\hyper@nd}%
                     \expandafter\ifx\csname hyperd@\meaning\hyper@t@mp@
                     \endcsname
                     \relax
                     \gdef#1{{}{\hyperstr@pquote#2"\hyper@nd}%
                               {\hyperstr@pquote#3"\hyper@nd}}%
                     \global\let\hyper@t@mp@=\relax
                     #4%
                     \else
		     \def\hyper@@tmp@{\hyper@nique{#1}{#2}}%
		     \edef\hyper@@tmp@@{{#3@}}%
                     \global\let\hyper@t@mp@=\relax
   		     \expandafter\hyper@@tmp@\hyper@@tmp@@{#4}%
                     \fi}}%

%%% 
% protection macros
%%%
\ifx\protect\hyper@ndefined\let\protect=\relax\fi
\let\hyper@@@@=\relax
\def\hyper@@{\let\hyper@@@=\relax}%
\hyper@@
\def\hyper@{\relax\let\hyper@@@\noexpand\hyper@\noexpand}%
\def\hyperpr@ref{\hyper@@\hyperref}
\def\hyperpr@link{\hyper@@\hyperlink}
\def\hyperpr@def{\hyper@@\hyperdef}
\let\hyper@marker=\relax
\def\hyper@@tokenize#1\hyper@marker{#1}
\def\hyper@tokenize{\expandafter\endgroup\hyper@@tokenize}
\def\hyperpr@tokenize{\hyper@@\hyper@tokenize}

% As per pg's suggestion
\edef\href{\begingroup\catcode`\string @=11
            \hyper@\hyperpr@tokenize\hyper@\hyperpr@link
            \hyper@marker}
\let\hname\hypertarget
% Hack to allow auto-processing
\def\allowoncemore{\def\hyper@utoprocess{\let\hyper@utoprocess=\hyper@ndefined
                                         \hypers@fe\endinput}}%
%
% Restore the catcode of @
%
\hypers@fe
\endinput
% A line after endinput to avoid both msdos gremlins and an incomplete
% last line

